When Raw Data Prevails: Are Large Language Model Embeddings Effective in Numerical Data Representation for Medical Machine Learning Applications?

The introduction of Large Language Models (LLMs) has advanced data representation and analysis, bringing significant progress in their use for medical questions and answering. Despite these advancements, integrating tabular data, especially numerical data pivotal in clinical contexts, into LLM paradigms has not been thoroughly explored. In this study, we examine the effectiveness of vector representations from last hidden states of LLMs for medical diagnostics and prognostics using electronic health record (EHR) data. We compare the performance of these embeddings with that of raw numerical EHR data when used as feature inputs to traditional machine learning (ML) algorithms that excel at tabular data learning, such as eXtreme Gradient Boosting. We focus on instruction-tuned LLMs in a zero-shot setting to represent abnormal physiological data and evaluating their utilities as feature extractors to enhance ML classifiers for predicting diagnoses, length of stay, and mortality. Furthermore, we examine prompt engineering techniques on zero-shot and few-shot LLM embeddings to measure their impact comprehensively. Although findings suggest the raw data features still prevails in medical ML tasks, zero-shot LLM embeddings demonstrate competitive results, suggesting a promising avenue for future research in medical applications.

==> embedding.tex <==


Table~\ref{tab:embedding_xgb} reveals that XGB stands out in diagnosing at Site X. At Site Y, LLMs like Mistral-7B-ins and Meditron demonstrate strong performances, with Mistral achieving scores of 71.11 and 55.71 for Sepsis and CHF, respectively. Llama2-13B and ClinicalBERT show competitive results, closely matching or even surpassing XGBoost in certain categories, especially noticeable in Llama2's performance in Arrhythmia with a score of 60.56. This comparison highlights the potential of LLMs in complex medical predictive modeling, underscoring their sophisticated language processing capabilities and their ability to closely compete with XGB, especially in external validation scenarios. 



\begin{table*}[ht]
\centering
\small 
\begin{tabular}{lllll}
\toprule
\textbf{Model}  & \textbf{Sepsis AUROC}  & \textbf{Arrhythmia AUROC}  & \textbf{CHF AUROC} & Average \\ 
& (95\% CI) & (95\% CI) & (95\% CI)& (95\% CI) \\
\midrule
\multicolumn{5}{c}{Machine Learning Baseline} \\ \midrule 
XGB & \textbf{71.17 (67.06, 75.11)} & \textbf{76.49 (71.32, 84.13)} & 58.47 (51.36, 65.15) & \textbf{68.71, (63.25, 74.80)} \\
ElasticNet &  71.10 (67.01, 75.18) & 74.40 (69.35, 79.56) & 54.79 (47.74, 61.79) & 66.76, (61.37, 72.18) \\
RandomForest &  65.26 (61.79, 68.48) & 53.07 (50.58, 55.80) & 50.89 (49.01, 53.43) & 56.41, (53.79, 59.24) \\
 \midrule
\multicolumn{5}{c}{LLM embedding + XGB classifier} \\ \midrule 
mistral & 71.12 (67.54, 74.92) & 67.29 (61.18, 72.75) & 51.80 (44.48, 58.65) & 63.40, (57.73, 68.77) \\
% & Notes & 56.53 (52.14, 60.86) & 51.55 (45.27, 57.34) & 51.25 (44.36, 57.47) & 53.11, (47.26, 58.56) \\
% & Tab+Notes & 60.63 (56.07, 64.78) & 64.17 (58.44, 69.81) & 52.95 (46.29, 59.76) & 59.25, (53.60, 64.78) \\
llama2-13b & 66.02 (61.64, 70.32) & 58.62 (52.62, 64.46) & 49.69 (48.83, 62.58) & 58.11, (54.36, 65.79) \\
% & Notes & 48.03 (43.80, 52.54) & 54.28 (47.77, 60.92) & 48.55 (41.19, 55.19) & 50.29, (44.25, 56.22) \\
% & Tab+Notes & 61.48 (56.88, 65.64) & 57.55 (52.15, 63.23) & 55.76 (49.13, 62.20) & 58.26, (52.72, 63.69) \\
meditron & 66.74 (62.30, 66.15) & 67.62 (61.84, 73.36) & 57.34 (50.69, 56.85) & 63.90, (58.28, 65.45) \\
% & Tab+Notes & 59.36 (54.94, 63.54) & 64.72 (58.80, 70.64) & 49.88 (43.07, 56.91) & 57.99, (52.27, 63.70) \\
% & Notes & 59.36 (54.94, 63.54) & 64.72 (58.80, 70.64) & 49.88 (43.07, 56.91) & 57.99, (52.27, 63.70) \\
clinicalBERT & 58.80 (54.44, 63.04) & 64.91 (61.84, 70.27) & 49.67 (41.94, 57.51) & 57.79, (52.74, 63.61) \\
% & Tab+Notes & 58.26 (53.70, 62.36) & 51.84 (45.12, 58.39) & 50.86 (44.20, 57.61) & 53.65, (47.67, 59.45) \\
% & Notes & 51.77 (46.94, 56.39) & 57.57 (51.30, 63.79) & 51.82 (45.14, 58.12) & 53.72, (47.79, 59.43) \\ 
 \midrule
\multicolumn{5}{c}{LLM embedding + ElasticNet classifier} \\ \midrule 
mistral & 62.61 (58.17, 66.95) & 69.59 (64.67, 74.71) & 48.98 (42.96, 55.62) & 60.39 (55.27, 65.76) \\ 
% & Notes & 49.65 (45.32, 54.04) & 52.61 (46.37, 58.77) & 49.06 (42.08, 55.66) \\
% & Tab+Notes & 53.28 (48.73, 57.69) & 59.62 (53.90, 65.11) & 49.11 (42.15, 55.46) \\
llama2-13b & 66.95 (62.82, 70.88) & 66.04 (60.04, 71.22) & \textbf{58.54 (52.09, 65.09)} & 63.84 (58.32, 69.06) \\  
% & Notes  & 46.02 (41.50, 50.14) & 47.36 (41.75, 53.41) & 46.99 (40.72, 53.19) \\ 
% & Tab+Notes & 54.20 (49.76, 58.61) & 61.80 (56.32, 67.39) & 51.54 (45.26, 57.82) \\
meditron &  66.91 (62.83, 71.09) & 68.61 (63.49, 73.72) & 57.60 (51.02, 63.89) & 64.37 (59.11, 69.90) \\  
% & Notes  & 46.96 (42.45, 51.59) & 44.67 (39.18, 50.07) & 46.70 (40.39, 52.64) \\
% & Tab+Notes & 46.73 (42.22, 51.01) & 44.75 (38.51, 50.65) & 46.79 (40.35, 53.31) \\
clinicalBERT & 47.28 (43.07, 51.63) & 44.62 (38.79, 50.29) & 46.98 (42.96, 55.62) & 46.29 (41.61, 52.51) \\ 
% & Notes  & 46.68 (42.41, 51.15) & 44.64 (38.74, 50.45) & 47.05 (40.52, 53.53) \\
% & Tab+Notes & 47.23 (42.83, 51.76) & 44.73 (38.74, 50.83) & 46.90 (40.53, 53.26) \\
\bottomrule
\end{tabular}
\label{tab:ml_baselines_sepsis_arrhythmia_chf_prediction}
\caption{ML baseline and LLM embedding with ML classifiers for Sepsis, Arrhythmia, and CHF Prediction}

\end{table*}


\subsection{Mortality Prediction Tasks}

\begin{table}[]
\small 
    \centering
    \begin{tabular}{llllll} \toprule 
       Model  & \multicolumn{2}{c}{mort ICU} & \multicolumn{2}{c}{mort Hosp}  \\ 
       & Acc. & AUROC & Acc. & AUROC \\ \midrule  
       LR & 93.4 & 88.70 & 91.1 & 85.6  \\ 
       RF & 93.3 & 89.7 & 90.7 & 86.7 \\
       XGB & \\ 
       \midrule 
       Mistral & 92.94 & 84.10 & 89.96 & 80.71 \\ 
       Meditron & 92.99 & 81.70 & 90.15 & 81.26 \\ 
    \end{tabular}
    \caption{Mortality prediction (\textcolor{red}{add in llama2}) }
    \label{tab:my_label}
\end{table}

\begin{table}[]
\small 
    \centering
    \begin{tabular}{llllll} \toprule 
       Model  & \multicolumn{2}{c}{LOS 3} & \multicolumn{2}{c}{LOS 7}  \\ 
       & Acc. & AUROC & Acc. & AUROC \\ \midrule  
       LR & 71.6 & 73.6 & 91.9 & 72.4  \\ 
       RF & 73.6 & 69.5 & 92.3 & 76.4 \\
       XGB & \\ 
       \midrule 
       Mistral & 65.91 & 68.39 & 92.34 & 72.36 \\ 
       Meditron & 66.62 & 69.78 & 92.34 & 69.51 \\ 
       \bottomrule 
    \end{tabular}
    \caption{Length-of-stay (\textcolor{red}{add in llama2})}
    \label{tab:my_label}
\end{table}

\section{Studies on LLM embedding representation}
\label{sec:llm_ablation}
In our study, we explore the effectiveness of language model embeddings in the context of medical diagnosis prediction by employing both mean and max pooling strategies. To assess these models, we utilize two distinct types of questions. The first, a general question type, asks, "What are the diagnoses of this patient?" aiming to gauge the model's overall diagnostic capability. The second, a "harness" type question, is more targeted, asking, "Does this patient have $\{target\_diagnosis\}$?" This approach allows us to compare the models' ability to provide broad diagnostic insights versus their precision in identifying specific conditions.

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{latex/Figs/model_emb_question.png}
    \caption{\small Does the question type and pooling method matter to the LLM embedding quality? (Probably add one without question type)}
    \label{fig:enter-label}
\end{figure*}
Our analysis reveals that max-pooling generally outperforms mean pooling across different models and question types, indicating a more effective aggregation of information for diagnosis prediction. As presented in Table~\ref{tab:emb_configuration}, Mistral-7B-Instruct with max pooling achieved notable success in the general question category, showcasing its robustness in broader diagnostic tasks. The comparison across question types indicates varying model preferences, yet the performance gap between the two types is minimal, leading us to choose the general type for our analysis.




\subsection{Few-shot on tabular data}

\begin{table}[ht]
\small 
\centering
\begin{tabular}{lllll}
\toprule
\textbf{Model} & \textbf{Shot Type} & \textbf{Sepsis} & \textbf{Arrhy.} & \textbf{CHF} \\
\midrule
Mistral & CoT & 64.29 & 64.35 & 57.32$\uparrow$ \\
llama2-13b & CoT & 62.12 & 63.96$\uparrow$ & 51.44$\uparrow$ \\
Meditron & CoT & 65.85$\uparrow$ & 64.29 & 52.90 \\
\bottomrule
\end{tabular}
\caption{Simple input-output few-shot (\textcolor{red}{Need to run this})} 
\label{tab:model_performance_fewshot}
\end{table}


\begin{table}[ht]
\small 
\centering
\begin{tabular}{lllll}
\toprule
\textbf{Model} & \textbf{Shot Type} & \textbf{Sepsis} & \textbf{Arrhy.} & \textbf{CHF} \\
\midrule
Mistral & CoT & 64.29 & 64.35 & 57.32$\uparrow$ \\
llama2-13b & CoT & 62.12 & 63.96$\uparrow$ & 51.44$\uparrow$ \\
Meditron & CoT & 65.85 & 64.29 & 52.90 \\
\bottomrule
\end{tabular}
\caption{Model Performance on Sepsis, Arrhythmia, and CHF Prediction using FewShot CoT (\textcolor{red}{Need to run multiple combos of CoT examples})}
\label{tab:model_performance_fewshot}
\end{table}



\subsection{Does system prompt help to improve the embedding for inst-based LLM?}
\begin{table}[h]
\small 
\centering
\begin{tabularx}{\columnwidth}{@{}cX@{}}
\toprule
\textbf{Setting} & \textbf{Description} \\
\midrule
Sys prompt1 & As a healthcare provider, please assess the patient's condition provided below and outline the likely causes or diagnoses for their clinical worsening. List only the diagnoses and keep your response brief. \\
\addlinespace
Sys prompt 2 & You are an AI with medical expertise. Create an embedding for the probable problems or diagnoses that are causing clinical deterioration, based on the patient's condition detailed below, to aid in training a diagnostic prediction machine learning classifier. Be brief in your description. \\
\addlinespace
Sys prompt 3 & As a medical expert, please examine the patient's condition by first identifying any abnormal values. Next, critically analyze these values to assess their impact, and clearly state your final diagnosis regarding what might be causing the clinical deterioration. Keep your summary brief. \\
\addlinespace 
Sys prompt 4 &You are a medical doctor. Based on the patient’s condition, determine the likelihood that diagnosis X is causing their clinical deterioration. Be aware that diagnosis X occurs in Y\% of similar cases.\\ 
\bottomrule
\end{tabularx}
\caption{System Prompts for Medical Diagnosis Assistance (lowest perplexity from paraphrases)}
\label{tab:prompts}
\end{table}

system prompt 1 vs 2: change of persona; system prompt 1 vs 3: think step-by-step; 


\begin{table}[h!]
\small 
    \centering
    \begin{tabular}{lllc}
    \toprule
    Model & Sys Type & Diagnosis & One-time AUROC (CI) \\
    \midrule
    Mistral & base & Sepsis & 0.7112 (0.6754, 0.7492) \\ 
    Mistral & Sys1 & Sepsis & 0.7135 (0.6690, 0.7553) \\
    Mistral & Sys2 & Sepsis & 0.6763 (0.6344, 0.7191) \\
    & Sys3 & Sepsis & 0.6567 (0.6130, 0.7006) \\ 
    & sys4 & Sepsis & 0.6787 (0.6346, 0.7173)) \\ 
     & base & Arrhythmia & 0.6729 (0.6118, 0.7275) \\
    Mistral & Sys1 & Arrhythmia & 0.6227 (0.5627, 0.6762) \\
    Mistral & Sys2 & Arrhythmia & 0.6384 (0.5805, 0.6960) \\
     Mistral & Sys3 & Arrhythmia & 0.6492 (0.5928, 0.7083) \\ 
     & base & CHF  & 0.5180 (0.4448, 0.5865) \\ 
    Mistral & Sys1 & CHF  & 0.5485 (0.4774, 0.6191) \\
    Mistral & Sys2 & CHF  & 0.5388 (0.4683, 0.6091) \\
    Mistral & Sys3 & CHF  & 0.5116 (0.4430, 0.5808) \\
    llama2-13b & base & Sepsis & 0.6602 (0.6164, 0.7032)\\
    llama2-13b & Sys1 & 0.6879 (0.6449, 0.7281) \\ 
     Llama2-13b & Sys2 & Sepsis & 0.6982 (0.6580, 0.7351) \\
    Llama2-13b & Sys3 & Sepsis & 0.6892 (0.6481, 0.7280) \\
         & base & Arrhythmia &  0.5862 (0.5262, 0.6446) \\ 
    Llama2-13b & Sys1 & Arrhythmia & 0.6924 (0.6326, 0.7509) \\
    Llama2-13b & Sys2 & Arrhythmia & 0.6190 (0.5625, 0.6764) \\
     Llama2-13b & Sys3 & Arrhythmia & 0.6144 (0.5549, 0.6658) \\
      & base & CHF & 0.4969 (0.4883, 0.6258) \\ 
    Llama2-13b & Sys1 & CHF  & 0.5649 (0.4937, 0.6305) \\
    Llama2-13b & Sys2 & CHF  & 0.5561 (0.4913, 0.6248) \\
    Llama2-13b & Sys3 & CHF & 0.5041 (0.4370, 0.5748) \\
    \bottomrule
    \end{tabular}
    \caption{AUROC Scores by model, system prompt yype, and diagnosis}
    \label{tab:auroc_scores}
\end{table}



==> features.tex <==
\paragraph{Embedding} To generate embeddings, we convert tabular data in natural language, as shown in Figure~\ref{fig:study_overview}, into parameters-frozen LLMs. After experimenting with various configurations, we find max pooling across token embeddings to be most effective, with detailed comparisons in the appendix \ref{sec:llm_ablation} through ablation studies on embedding techniques. These embeddings are then input into an XGB classifier for diagnosis prediction training. 

XGB with raw data inputs serves as our baseline. Besides Mistral and Llama2, we include Meditron-7B~\cite{chen2023meditron}, a Llama2-based model pre-trained on the medical corpus. We also include ClinicalBERT~\cite{alsentzer2019publicly}, which is trained on public EHR data from a different site as a comparison to decoder-only models.  

\paragraph{A/B token probability} We focus on the answer option \textsc{a} and \textsc{b} token probabilities, where they correspond to \textsc{yes} and \textsc{no} options, respectively, gauging their confidence in making binary decisions. To calculate, we add a diagnostic question to our input (see Figure~\ref{fig:study_overview}) and extract the softmax probabilities for  from the model's output. We further normalize their probabilities by their sum to a scale of 0 and 1, excluding the distribution probabilities of other vocabulary terms in the model.   

\paragraph{Answer sequence likelihood} 
%Examining the log-likelihood of full answer sequences offers a detailed perspective on the model's reasoning process, revealing how it synthesizes contextual details and prior knowledge to conclude. 
Calculating answer sequence likelihood yields a contextualized representation, highlighting the model's ability to integrate given context and prior knowledge into its reasoning. We append the answer choice ``A. Yes.'' and ``B. No.'' to the input text and question. The resulting sequences are fed into LLM and we extract the log probability of the answer sequence following previous work~\cite{ren2023self}, where $x$ is input and $y_t$ are the answer tokens: 
\begin{equation}
\small 
\vspace{-.18in}
    \log p(y|x) = \sum_{t=1}^{l} \log p(y_t | y_1, \ldots, y_{t-1}, x).
\end{equation}


==> full_table.tex <==

\begin{table*}[ht]
\centering
\small 
\begin{tabular}{lllll}
\toprule
\textbf{Model} & \textbf{Input Type} & \textbf{Sepsis AUROC}  & \textbf{Arrhythmia AUROC}  & \textbf{CHF AUROC}  \\ 
& & (95\% CI) & (95\% CI) & (95\% CI) \\
\midrule
\multicolumn{5}{c}{Machine Learning Baseline} \\ \midrule 
XGB 
 & BoC & 63.20 (62.89, 63.50) & 63.37 (62.45, 64.30) & 46.15 (45.48, 46.82) \\
 & Tab & 72.88 (72.39, 73.38) & 71.06 (70.43, 71.70) & - \\
 & Tab+BoC & 60.89 (60.48, 61.30) & 63.13 (62.78, 63.48) & - \\
ElasticNet 
 & BoC & 58.80 (54.22, 63.17) & 56.15 (49.70, 62.63) & 43.82 (36.37, 51.58) \\
 & Tab & 71.10 (67.01, 75.18) & 74.40 (69.35, 79.56) & 54.79 (47.74, 61.79) \\
 & Tab+BoC & 72.79 (68.82, 76.61) & 74.10 (69.17, 78.95) & 58.91 (52.17, 65.77) \\
RandomForest 
 & BoC & 58.69 (55.58, 61.87) & 54.01 (51.37, 57.12) & 52.09 (49.55, 55.04) \\
 & Tab & 65.26 (61.79, 68.48) & 53.07 (50.58, 55.80) & 50.89 (49.01, 53.43) \\
 & Tab+BoC & 68.34 (64.82, 71.73) & 50.50 (49.03, 52.49) & 53.89 (50.94, 57.35) \\
 \midrule
\multicolumn{5}{c}{LLM embedding + XGB classifier} \\ \midrule 
mistral & Tab & 71.12 (67.54,74.92) & 67.29 (61.18, 72.75) & 51.80 (44.48, 58.65) \\ 
& BoC & - & - & - \\
 & Tab+BoC & 60.39 (55.58, 65.64) & 59.25 (52.75, 66.14) & 56.58 (48.41, 64.24) \\
 & Notes Only & 56.53 (52.14, 60.86) & 51.55 (45.27, 57.34) & 51.25 (44.36, 57.47) \\
 & Tab+Notes & 60.63 (56.07, 64.78) & 64.17 (58.44, 69.81) & 52.95 (46.29, 59.76) \\
llama2-13b & Tab & 66.02 (61.64, 70.32) & 58.62 (52.62, 64.46) & 49.69 (48.83, 62.58)\\  
& BoC & - & - & - \\
 & Tab+BoC & 59.42 (54.53, 64.70) & 57.52 (50.98, 63.98) & 59.02 (51.04, 66.98) \\
 & Notes Only & 48.03 (43.80, 52.54) & 54.28 (47.77, 60.92) & 48.55 (41.19, 55.19) \\
 & Tab+Notes & 61.48 (56.88, 65.64) & 57.55 (52.15, 63.23) & 55.76 (49.13, 62.20) \\
meditron & Tab &  66.74 (62.30, 66.15) & 67.62 (61.84, 73.36) & 57.34 (50.69, 56.85)\\ 
& CUI Only & 50.80 (46.27, 55.32) & 55.76 (50.02, 61.76) & 55.97 (48.74, 62.92) \\
 & Tab+BoC & 58.25 (53.87, 62.51) & 64.68 (59.14, 69.97) & 57.58 (50.58, 64.41) \\
 & Tab+Notes & 59.36 (54.94, 63.54) & 64.72 (58.80, 70.64) & 49.88 (43.07, 56.91) \\
  & Notes Only & 59.36 (54.94, 63.54) & 64.72 (58.80, 70.64) & 49.88 (43.07, 56.91) \\ 
clinicalBERT & 58.80 (54.44, 63.04) & 64.91 (61.84, 70.27) & 49.67 (41.94, 57.51)\\ 
& CUI Only & 53.89 (49.29, 58.22) & 54.27 (47.98, 61.02) & 55.29 (48.25, 61.73) \\
 & Tab+BoC & 59.12 (54.66, 63.76) & 59.64 (53.17, 65.69) & 52.48 (45.38, 58.98) \\
 & Tab+Notes & 58.26 (53.70, 62.36) & 51.84 (45.12, 58.39) & 50.86 (44.20, 57.61) \\
& Notes Only & 51.77 (46.94, 56.39) & 57.57 (51.30, 63.79) & 51.82 (45.14, 58.12) \\ 
\midrule 
\multicolumn{5}{c}{LLM embedding + ElasticNet classifier} \\ \midrule 
mistral & Tab & \\ 
& BoC & 59.10 (54.53, 63.53) & 46.02 (39.77, 51.69) & 41.23 (34.55, 48.07) \\
 & Tab+BoC & 60.13 (55.78, 64.64) & 54.42 (48.13, 60.56) & 42.01 (35.66, 49.34) \\
 & Tab+Notes & 53.28 (48.73, 57.69) & 59.62 (53.90, 65.11) & 49.11 (42.15, 55.46) \\
 & Notes Only & 49.65 (45.32, 54.04) & 52.61 (46.37, 58.77) & 49.06 (42.08, 55.66) \\
llama2-13b & Tab & \\  
& BoC & 50.08 (45.76, 54.31) & 48.31 (42.05, 55.12) & 42.86 (36.37, 48.74) \\
 & Tab+BoC& 60.19 (55.67, 64.28) & 66.14 (59.64, 71.39) & 43.02 (36.85, 49.67) \\
 & Tab+Notes & 54.20 (49.76, 58.61) & 61.80 (56.32, 67.39) & 51.54 (45.26, 57.82) \\
 & Notes Only & 46.02 (41.50, 50.14) & 47.36 (41.75, 53.41) & 46.99 (40.72, 53.19) \\ 
meditron & Tab & \\  
& BoC & 42.88 (38.59, 47.08) & 45.43 (39.49, 51.74) & 47.28 (40.27, 54.13) \\
 & Notes Only & 46.96 (42.45, 51.59) & 44.67 (39.18, 50.07) & 46.70 (40.39, 52.64) \\
 & Tab+BoC & 43.54 (39.29, 48.15) & 50.71 (44.40, 56.77) & 47.60 (41.28, 54.10) \\
 & Tab+Notes & 46.73 (42.22, 51.01) & 44.75 (38.51, 50.65) & 46.79 (40.35, 53.31) \\
clinicalBERT & Tab & \\ 
& BoC & 43.19 (38.65, 47.66) & 42.30 (36.52, 48.44) & 43.39 (36.85, 49.74) \\
 & Tab+BoC & 43.54 (39.00, 47.81) & 42.28 (36.91, 47.88) & 43.32 (36.72, 49.94) \\
 & Tab+Notes & 47.23 (42.83, 51.76) & 44.73 (38.74, 50.83) & 46.90 (40.53, 53.26) \\
 & Notes Only & 46.68 (42.41, 51.15) & 44.64 (38.74, 50.45) & 47.05 (40.52, 53.53) \\
\bottomrule
\end{tabular}
\label{tab:ml_baselines_sepsis_arrhythmia_chf_prediction}
\caption{ML baseline and LLM embedding with ML classifiers for Sepsis, Arrhythmia, and CHF Prediction}

\end{table*}


\begin{table}[h!]
\small 
    \centering
    \begin{tabular}{lllc}
    \toprule
    Model & Sys Type & Diagnosis & One-time AUROC (CI) \\
    \midrule
   Of all models & Best & Sepsis & 0.7117 (0.6706, 0.7511) \\ 
    Mistral & base & Sepsis & 0.7112 (0.6754, 0.7492) \\ 
     & Sys1 & Sepsis & 0.7135 (0.6690, 0.7553) \\
     & Sys2 & Sepsis & 0.6763 (0.6344, 0.7191) \\
    & Sys3 & Sepsis & 0.6567 (0.6130, 0.7006) \\ 
    & sys4 & Sepsis & 0.6787 (0.6346, 0.7173)) \\
    Of all models & Best & Arrhythmia & 0.7649 (0.7132, 0.8413) \\ 
   Mistral  & base & Arrhythmia & 0.6729 (0.6118, 0.7275) \\
     & Sys1 & Arrhythmia & 0.6227 (0.5627, 0.6762) \\
     & Sys2 & Arrhythmia & 0.6384 (0.5805, 0.6960) \\
      & Sys3 & Arrhythmia & 0.6492 (0.5928, 0.7083) \\ 
     & Sys4 & Arrhythmia & 0.6611 (0.6055, 0.7129) \\ 
   Of all models   & Best & CHF & 0.5854 (0.5209, 0.6509) \\ 
    Mistral & base & CHF  & 0.5180 (0.4448, 0.5865) \\ 
     & Sys1 & CHF  & 0.5485 (0.4774, 0.6191) \\
     & Sys2 & CHF  & 0.5388 (0.4683, 0.6091) \\
     & Sys3 & CHF  & 0.5116 (0.4430, 0.5808) \\
    & Sys4 & CHF & 0.5404  (0.4752, 0.6102) \\  
    llama2-13b & base & Sepsis & 0.6602 (0.6164, 0.7032)\\
     & Sys1 & Sepsis& 0.6879 (0.6449, 0.7281) \\ 
     & Sys2 & Sepsis & 0.6982 (0.6580, 0.7351) \\
     & Sys3 & Sepsis & 0.6892 (0.6481, 0.7280) \\
    & Sys4 & Sepsis & 0.6462 (0.6031, 0.6883) \\
       Llama2-13b   & base & Arrhythmia &  0.5862 (0.5262, 0.6446) \\ 
    & Sys1 & Arrhythmia & 0.6924 (0.6326, 0.7509) \\
     & Sys2 & Arrhythmia & 0.6190 (0.5625, 0.6764) \\
      & Sys3 & Arrhythmia & 0.6144 (0.5549, 0.6658) \\
     & Sys4 & Arrhythmia & 0.6443 (0.5832, 0.6992) \\ 
    Llama2-13b  & base & CHF & 0.4969 (0.4883, 0.6258) \\ 
     & Sys1 & CHF  & 0.5649 (0.4937, 0.6305) \\
     & Sys2 & CHF  & 0.5561 (0.4913, 0.6248) \\
     & Sys3 & CHF & 0.5041 (0.4370, 0.5748) \\
    & Sys4 & CHF & 0.6024 (0.5307, 0.6664)) \\ 
    Meditron & base & Sepsis & \\ 
    & Sepsis & Sys1 &  0.6728 (0.6323, 0.7123) \\
    & Sepsis & Sys2 & 0.6728  (0.6301, 0.7093) \\ 
    &Sepsis & Sys3&  0.6728  0.6285, 0.7165 \\ 
    &Sepsis & Sys4 & 
    \bottomrule
    \end{tabular}
    \caption{AUROC Scores with 95\% confidence intervals by model, system prompt type, and diagnosis}
    \label{tab:auroc_scores}
\end{table}


==> methods.tex <==




\section{LLMs for Diagnosis Generation with Natural Language Output}
\label{sec:nl_output}
%\input{probing}

\begin{table}[ht]
\small 
    \centering
    \begin{tabular}{c c c c} \toprule
       Model  & Range & Units & Reasoning \\ \midrule
        Mistral & 4.25$\pm$0.99 & 4.26$\pm$0.86 &  4.83$\pm$0.65 \\ 
        Llama2 & 3.92$\pm$1.10 & 4.71$\pm$0.93 & 3.27$\pm$1.08 \\ \bottomrule
    \end{tabular}
    \vspace{-.1in}
    \caption{\small Physician evaluation on the Mistral and Llama2 probing output. Examples can be found in the Appendix \S \ref{sec:prob_examples}.}
    \label{tab:probing}
\end{table}

We employ two mainstream instruction-finetuned LLMs, Mistral-7B-instruct~\cite{jiang2023mistral} (Mistral) and Llama2-13B-Chat (Llama2)~\cite{touvron2023llama}. The first task assesses LLMs' understanding of measurement units and reference ranges for 24 vital signs and laboratory results. A board-certified physician evaluates the outputs on a 1 to 5 Likert scale across three categories: correct range, measurement units, and explanation quality ("Reasoning"). Table~\ref{tab:probing} summarizes the findings, with Mistral outperforming Llama2, especially in identifying normal ranges and providing explanations, scoring 4.25 and 4.83 versus Llama2's 3.92 and 3.27, respectively. These results highlight LLMs' inherent knowledge of physiological data ranges, suggesting their potential utility in medical context.

%We apply two LLMs on this set of tasks: Mistral-7B-instruct~\cite{jiang2023mistral} (Mistral), Llama2-13B-Chat (Llama2), both of which are NLP leaderboard winners and finetuned towards instructions. The first task is to probe LLM for their internal knowledge about physiological data. We prompt the LLM for its understanding of the measurement units and reference ranges for the same 24 vital signs and laboratory results from the collected . A board-certified physician then evaluates the output using a Likert scale of 1 to 5 on the three categories (strongly disagree to strongly agree): correct range, units of measurement, and quality of explanations provided (``Reasoning''). The findings are summarized in Table~\ref{tab:probing}. Mistral outperforms Llama2 in accurately identifying normal ranges and providing explanations, scoring 4.25 and 4.83 against Llama2's 3.92 and 3.27 in these categories, respectively. The results suggest that the LLMs possess inherent knowledge of the numerical ranges of physiological data, indicating their potential utility in medical contexts. 

 On the diagnosis generation task, we implement a self-consistency setting, where the same answer sets are shuffled multiple times with different orderings. This helps to mitigate the potential bias introduced by the ordering of answer options~\cite{ren2023self}. For a given question, the answer set includes the true diagnoses as well as other diagnoses. There are 3 self-consistency examples per input, and we measure the average exact match per input as performance evaluation. Table~\ref{tab:mul_qa} presents the results using Mistral and Llama2. Overall, Mistral achieves higher exact match (EM) scores compared to Llama2 at both Site X (43.69\% vs. 28.79\%) and Site Y (27.33\% vs. 20.67\%). 


\begin{table}[ht]
\small 
\centering
\begin{tabular}{l l l l l}
\toprule 
Model             & Site & EM    & Site & EM   \\ \midrule
random  & X & 27.78 & Y & 22.47 \\  
Mistral-7B-ins    & X   & 43.69 & Y   & 27.33 \\ 
Llama2-13b-chat   & X   & 28.79 & Y   & 20.67 \\ \bottomrule
\end{tabular}
\vspace{-.1in}
\caption{\small Model performance (evaluated by exact match) on the Multiple QA task. We add a `Random` baseline to serve as a foundational comparison point.}
\label{tab:mul_qa}
\end{table}



\begin{table*}[h]
\small 
\centering
\begin{tabular}{l c c c c  c c c c }
\toprule
& \multicolumn{4}{c}{Site X} & \multicolumn{4}{c}{Site Y} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9}
Model & Sepsis & Arrhy. & CHF & Average & Sepsis & Arrhy. & CHF & Average \\
\midrule
\multirow{2}{*}{XGB} & \textbf{72.35}& \textbf{76.48} & \textbf{58.49} & \textbf{69.10} & \textbf{62.66} & 56.06 & \textbf{55.55} & \textbf{58.09} \\ 
\multirow{2}{*}{ElasticNet} & \textbf{72.35}& \textbf{76.48} & \textbf{58.49} & \textbf{69.10} & \textbf{62.66} & 56.06 & \textbf{55.55} & \textbf{58.09} \\ 
\multirow{2}{*}{SVM} \\ 
\multirow{2}{*}{RandomForest} \\ 
& \scriptsize{71.02, 77.11} & \scriptsize{74.37, 86.48} & \scriptsize{46.97, 60.28} & \scriptsize{64.12, 74.96} & \scriptsize{59.01, 68.23} & \scriptsize{46.69, 57.02} & \scriptsize{47.87, 59.49} & \scriptsize{51.19,61.91} \\ \midrule 
Mistral & 71.11 & 67.05 & 55.71 & 64.62 & 55.52 & 52.48 & 54.82 & 54.16 \\
& \scriptsize{70.83, 76.92} & \scriptsize{57.77, 69.92} & \scriptsize{52.49, 65.86} & \scriptsize{60.03, 70.57}  & \scriptsize{52.61, 61.81} & \scriptsize{50.10, 59.64} & \scriptsize{45.32, 57.96} &  \scriptsize{49,34, 59.14} \\
Llama2 & 63.87 & 58.60 & 49.69 & 57.39 & 54.56 & \textbf{60.56} & 50.45 & 55.19 \\
& \scriptsize{60.24, 68.74} & \scriptsize{52.25, 64.43} & \scriptsize{41.08, 54.80} & \scriptsize{51.19, 62.32} & \scriptsize{50.04, 59.22} & \scriptsize{57.89, 68.19} & \scriptsize{48.92, 63.09} & \scriptsize{52.28, 63.50} \\
Meditron & 66.67 & 67.61 & 57.34 & 63.87 & 52.16 & 54.07 & 48.43 & 51.55 \\
& \scriptsize{62.94, 70.46} & \scriptsize{65.82, 77.90} & \scriptsize{50.17, 62.29} & \scriptsize{59.31,70.55} & \scriptsize{47.21, 56.38} & \scriptsize{52.27, 62.18} & \scriptsize{46.03, 58.54} & \scriptsize{48.83, 59.37} \\
ClinicalBERT & 58.82 & 64.90 & 51.80 & 58.51 & 53.33 & 54.47 & 52.40 & 53.41 \\
& \scriptsize{59.83, 67.26} & \scriptsize{54.28, 66.22} & \scriptsize{44.32, 57.24} & \scriptsize{52.81, 63.24} & \scriptsize{46.94, 56.89} & \scriptsize{47.43, 59.39} & \scriptsize{47.41, 57.16} & \scriptsize{47.26, 57.48} \\
\bottomrule 
\end{tabular}
\vspace{-.12in}
\caption{\small AUROC scores and confidence intervals at Site X and external validation Site Y, where we test XGB classifier trained on site X for generalizability. Given that XGB baseline achieves high AUROC scores on Site X Sepsis and Arrhy. of 72.35 and 76.48, we leverage these two sets of XGB results for experiments in Table~\ref{tab:prob_corr}. Training details are included in Appendix \S \ref{sec:xgb_training}.  }
\label{tab:embedding_xgb}
\end{table*}


\section{LLMs for Feature Extraction in Diagnosis Classification} 
\label{sec:classification}

\subsection{Motivation} 
Probabilistic outputs from predictive models are vital for medical diagnostics, enhancing the understanding of diagnostic uncertainty and patient risk~\cite{chen2021probabilistic,hassan2023road}. Their precision, especially their alignment with evaluation frameworks like AUROC and calibration plots, is crucial for impacting clinical outcomes~\cite{la2019interpretation,hou2020predicting}. However, our initial analyses lack a thorough examination of these essential metrics, presenting a gap underscoring the need for an in-depth investigation into how model-generated probabilities fulfill medical diagnostics' stringent requirements. %Therefore, this section aims to scrutinize the discrimination and calibration capabilities of these probabilistic outputs, ensuring they adhere to medical decision-making standards. 

This section formulates the task as a binary diagnostic outcome classification using three LLMs feature extraction methods. We benchmark against XGB using raw features, correlating each method. Initially, LLM-derived embeddings are directly fed into the XGB classifier for training and testing. For the probability-based methods, we begin by correlating LLM probabilities with XGB's raw features trained from scratch. After establishing this baseline, we input these probabilities into the XGB classifier to observe any enhancements in their alignment. This setting allows us to fit LLMs within the established framework that prioritizes AUROC and calibration for medical decision-making.

\subsection{LLMs for tabular data feature representation}
\input{features}


\subsection{XGB classifier training details}
\label{sec:xgb_training}
The training process of the XGB classifier involved a systematic 5-fold cross-validation technique, ensuring a comprehensive assessment of the model's predictive power across the entire dataset. Each fold was used to train and validate a distinct segment of the data, mitigating the risk of overfitting and promoting the generalizability of our findings. On site X, each fold of the training set contains 528 data records, and test set size is 132. On Site Y, the entire dataset is used as test set with 483 samples.  

During the training phase, we harnessed a grid search algorithm to fine-tune hyperparameters, identifying the optimal configuration for the XGBoost classifier. The best parameters were then utilized to train the model, which was further accelerated by exploiting GPU capabilities, notably decreasing the training time while handling the intricate calculations efficiently.

Finally, we evaluated the classifier's performance on the test set, obtaining the AUROC scores as our primary metric. In the external validation scenario, we used the entire site Y set as the test set. This score provides an aggregate measure of the model's ability to differentiate between the classes of interest. The classifier's predictive probabilities were also meticulously examined to enhance our understanding of the model's decision-making process.

All experiments are running on one A100 80GB GPU. Each LLM embedding + XGB experiment takes around 125 minutes. Each probing and multiple QA samples on LLM takes 2 minutes. 

We used python package sklearn for the performance metrics, which include: AUROC, calibration curve, Spearman correlation and Pearson correlation.  

\section{Studies on LLM embedding representation}
\label{sec:llm_ablation}
In our study, we explore the effectiveness of language model embeddings in the context of medical diagnosis prediction by employing both mean and max pooling strategies. To assess these models, we utilize two distinct types of questions. The first, a general question type, asks, "What are the diagnoses of this patient?" aiming to gauge the model's overall diagnostic capability. The second, a "harness" type question, is more targeted, asking, "Does this patient have $\{target\_diagnosis\}$?" This approach allows us to compare the models' ability to provide broad diagnostic insights versus their precision in identifying specific conditions.

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{latex/Figs/model_emb_question.png}
    \caption{\small Does the question type and pooling method matter to the LLM embedding quality? (Probably add one without question type)}
    \label{fig:enter-label}
\end{figure*}
Our analysis reveals that max-pooling generally outperforms mean pooling across different models and question types, indicating a more effective aggregation of information for diagnosis prediction. As presented in Table~\ref{tab:emb_configuration}, Mistral-7B-Instruct with max pooling achieved notable success in the general question category, showcasing its robustness in broader diagnostic tasks. The comparison across question types indicates varying model preferences, yet the performance gap between the two types is minimal, leading us to choose the general type for our analysis.



\begin{table}[ht]
\small 
    \centering
    \begin{tabular}{l c c c c c c}
    \toprule 
       \multirow{2}{*}{Model}  & \multirow{2}{*}{Dx} &  \multicolumn{2}{c}{Raw Prob} &  \multicolumn{2}{c}{w/ XGB}  \\
       & & $\rho$ & $r$ & $\rho$ & $r$ \\ \midrule
       \multicolumn{6}{c}{Embedding +XGB raw probability } \\  \midrule 
       Mistral  &  Sepsis & 0.542$^{*}$ & 0.571$^{*}$ & - & - \\ 
         &  Arrhy. & 0.288$^{*}$ & 0.323$^{*}$ & - & - \\  
         Llama2 & Sepsis & 0.510$^{*}$ & 0.543$^{*}$ & - & - \\ 
         & Arrhy. & 0.237$^{*}$ & 0.201$^{*}$ & - & - \\ 
       \midrule  
       \multicolumn{6}{c}{Token-based probability } \\ 
       \midrule 
       Mistral  &  Sepsis & 0.101 &  0.111$^{*}$ & <0 & <0 \\ 
       &  Arrhy. & <0 & <0  & 0.113$^{*}$ & 0.086$^{*}$ \\ 
       Llama2  &   Sepsis & 0.090$^{*}$ & 0.092$^{*}$ & 0.086$^{*}$ & 0.086$^{*}$  \\ 
       &   Arrhy. & <0  & <0 & 0.055 & 0.044\\ 
    	\midrule  
           \multicolumn{6}{c}{ Answer sequence likelihood } \\
	\midrule  
       Mistral  &  Sepsis & 0.024 & 0.021 &  0.03 & 0.04  \\ 
       &  Arrhy. & <0 & <0 &  0.003 & <0  \\ 
       Llama2  &  Sepsis & <0 & <0   & 0.136 & 0.123\\ 
        &  Arrhy. & <0 & <0   & <0 & 0.014\\  
       \bottomrule 
    \end{tabular}
    \vspace{-.12in}
    \caption{\small Spearman ($\rho$) and Pearson correlations ($r$) between the raw A/B token probabilities and XGB probabilities, and between the answer sequence probability and the raw XGB probabilities, with $^{*}$ denoting significant correlation (p-value <0.05). The AUROC scores of probability-based methods are presented in Appendix \S \ref{sec:prob_auroc}. }
    \label{tab:prob_corr}
\end{table}

Table~\ref{tab:embedding_xgb} reveals that XGB stands out in diagnosing at both sites. On site X, Mistral and Meditron show strong performance with confidence interval overlapping with XGB baseline on Sepsis, CHF, with Mistral achieving high AUROC scores of 71.11 compared to XGB baseline at 72.55. In the external validation at site Y, all models show reduced performance. Llama 2 and ClinicalBERT closely compete with XGB, particularly in Arrhythmia, where Llama 2's score of 60.56 surpasses XGB's 56.06. 
This comparison highlights LLMs' potential in medical predictive modeling, particularly against XGB in external validations.

Table~\ref{tab:prob_corr} presents the Spearman ($\rho$) and Pearson ($r$) correlation results of the two best-performing LLMs (Mistral and Llama2) from Table~\ref{tab:embedding_xgb}. We compare combined embeddings and XGB probabilities, token probabilities, and answer sequence probabilities with XGB's for Sepsis and Arrhythmia. On the combination of embedding with XGB, Mistral and Llama2 show moderate to strong correlations in Sepsis and Arrhythmia, with statistical significance. Token probabilities correlate weakly or inversely, especially without XGB, while answer sequence likelihoods show minimal correlation, indicating little to no linear relationship with XGB's predictions.
 This analysis reinforces the potential of LLM embeddings as promising representations for tabular data in medical diagnosis, yet it also underscores the unreliability of LLM probabilities as standalone predictive measures.


==> probing.tex <==

\begin{table}[ht]
    \centering
    \begin{tabular}{c|c c }
       Model  & Range & Units of Measurement  \\
       Mistral-7B  & \\ 
       Llama2-13B & \\ 
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}

==> rq0_probing.tex <==









==> rq2_influence.tex <==
\section{RQ2: Does prompt engineering help to improve LLM embeddings?}
 \label{sec:rq2} 





\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{latex/Figs/mistral_prompt_exps.png}
    \includegraphics[width=\textwidth]{latex/Figs/llama_prompt_exps.png}
    \vspace{-.28in}
    \caption{\small AUROC Scores with 95\% confidence intervals by model, system prompt type, and diagnosis. We compare the results from prompt-engineering with ``base'' results, which is the model with XGB results in table~\ref{tab:ml_baselines_sepsis_arrhythmia_chf_prediction}. Meditron is not an instruction-tuned model, therefore is not sensitive to the prompt and results were not included.  }
    \label{fig:prompt_impact}
\end{figure*}


% Given that LLMs are known to be sensitive to prompting, we suspect that the nature of the prompt will significantly impact the LLM embeddings. To investigate this, we test a set of four prompts that vary by persona, thinking style, and question type, enabling us to explore the influence of prompt characteristics on the embeddings and assess the model's robustness and adaptability across a variety of scenarios. 

% Our prompt engineering strategy follows previous work demonstrating the use of perplexity to select optimal prompts~\cite{gonen2023demystifying}. We first create meta-language prompts designed to specify the clinical scenarios and tasks. We then employ GPT-4, a leading LLM, to produce five distinct paraphrases for each initial prompt, aiming to explore a range of expressions and structures. For each paraphrase, we calculate the perplexity score to measure how well a probability model predicts a sample and is used here to gauge the naturalness and fluency of the text. Finally, the paraphrase with the lowest perplexity is selected for each meta-prompt as the final prompt for our experiments. This ensures that the prompts we use are the ones the language model finds most coherent, which is critical for the reliability of the system’s performance in subsequent diagnostic tasks. 

Experiment results from the Mistral and Llama2-13b models, as shown in Figure~\ref{fig:prompt_impact}, revealed how different prompt personas, question types, and thinking styles affect LLM performance in diagnosis prediction. Note that Meditron was not fine-tuned with instructions, so we observed no changes from this prompt-engineering experiment. Simple prompts that specify the persona of medical experts and the task (Prompt 1), along with binary question prompts that incorporate prevalence data (Prompt 4), generally achieved higher AUROCs. 
Mistral using prompt 1 achieved an AUROC of 71.35 for Sepsis prediction, and Llama2 with prompt 4 reached 60.24 for CHF, setting new highs and outperforming other models. The AI system persona (Prompt 2) and step-by-step thinking (Prompt 3) displayed more variable performance. The ability of prompt tuning to improve zero-shot performance indicates that LLMs can generate useful embeddings for ML tasks through prompt modifications. 

Prompt-engineering showed no significant improvements in mortality prediction and LOS tasks. For instance, Mistral's LOS 3 AUROC ranged from 66.13 to 68.55 across prompts 1, 2, and 3, comparable to its non-prompted zero-shot AUROC of 68.39 (see Figure~\ref{fig:mort_los}). This underscores the need for LLMs to improve representation of time-varying features.



==> rq3_fewshot.tex <==

\section{RQ3: Results from Few-shot Experiments}
 \label{sec:rq3}
% This research question investigates whether few-shot learning can enhance LLM embeddings by using synthetic examples generated from GPT-4. We focus our study on the diagnosis prediction use case, which involves relatively short inputs with 24 clinical features. This is in contrast to the more complex MIMIC-Extract dataset, which includes 104 features and 24 data points per feature, making it more challenging to verify the quality of synthetic data generation.  

% Specifically, we generate synthetic data representing patient cases with clinical deterioration, using the template in Table~\ref{tab:feat_and_templates}. These include a case where a diagnosis is confirmed (positive) and one where it is absent (negative). A expert physician and clinical informaticist reviews this synthetic data pair for quality assurance. We then conduct two sets of few-shot experiments. In the first, we slightly modify Prompt 1 by incorporating example input-output pairs, namely the ``Simple'' few-shot setting. In the second experiment, we instruct GPT-4 to generate a Chain-of-Thought (CoT) explanation detailing why the case is diagnosed as positive or negative. This CoT explanation is structured into three parts: identification of abnormal values, reasoning over these values, and concluding the diagnosis. We then integrate these CoT examples into Prompt 4. 



% \begin{table}[ht]
% \small 
% \centering
% \begin{tabular}{lllll}
% \toprule
% \textbf{Model} & \textbf{Shot Type} & \textbf{Sepsis} & \textbf{Arrhy.} & \textbf{CHF} \\
% \midrule
% Mistral & Simple & 67.32 & 68.43$\uparrow$ & 54.43 \\
% llama2-13b & Simple & 66.49$\uparrow$ & 67.74$\uparrow$ & 53.12$\uparrow$ \\
% Meditron & Simple & 67.28$\uparrow$ & 65.25 & 51.76 \\
% \midrule
% Mistral & CoT & 64.29 & 64.35 & 57.32$\uparrow$ \\
% llama2-13b & CoT & 62.12 & 63.96$\uparrow$ & 51.44$\uparrow$ \\
% Meditron & CoT & 65.85 & 64.29 & 52.90 \\
% \bottomrule
% \end{tabular}
% \vspace{-.1in}
% \caption{\small Model Performance on Sepsis, Arrhythmia, and CHF Prediction using few-shot examples. The upper arrows $\uparrow$ suggest there are improvements over the models' zero-shot non-prompting counterparts.}
% \label{tab:model_performance_fewshot}
% \end{table}


\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{latex/Figs/model_fewshot.png}
    \vspace{-.28in}
    \caption{\small When comparing to the non-prompted zero-shot LLM+XGB results in Table~\ref{tab:ml_baselines_sepsis_arrhythmia_chf_prediction}, AUROC and percentage improvements from few-shot types (Simple and CoT) on diagnosis prediction tasks. }
    \label{fig:model_performance_fewshot}
\end{figure}

Figure~\ref{fig:model_performance_fewshot} presents the AUROC and percentage improvements from the two few-shot settings, with varying levels of improvement across different models and target diagnosis. In the "Simple" shot type, Mistral, Llama2-13b, and Meditron showed modest gains in AUROC for diagnoses such as Sepsis and Arrhythmia, with Llama2-13b marking a noticeable improvement (15.3\%) across all its tested diagnoses. For the CoT approach, while the gains are less consistent, notable increases are observed particularly in CHF predictions for Mistral and Llama2-13b. This suggests that integrating few-shot learning approach can enhance the predictive performance of LLMs embeddings.  
